Annealed Co-Generation: Disentangling Variables via Progressive Pairwise Modeling

For multivariate co-generation in scientific applications, we advocate pairwise block rather than joint modeling of all variables. This design mitigates the computational burden and data imbalance. To this end, we propose an Annealed Co-Generation (ACG) framework that replaces high-dimensional diffusion modeling with a low-dimensional diffusion model, which enables multivariate co-generation by composing pairwise variable generations. We first train an unconditional diffusion model over causal variables that are disentangled into pairs. At inference time, we recover the joint distribution by coupling these pairwise models through shared common variables, enabling coherent multivariate generation without any additional training. By employing a three-stage annealing process-Consensus, Heating, and Cooling-our method enforces consistency across shared common variables and progressively constrains each pairwise data distribution to lie on a learnable manifold, while maintaining high likelihood within each pair. We demonstrate the framework's flexibility and efficacy on two distinct scientific tasks: flow-field completion and antibody generation. All datasets and code will be made publicly available upon publication.

==> algorithms/bubble-sort.tex <==
\begin{algorithm}[tb]
  \caption{Bubble Sort}
  \label{alg:example}
  \begin{algorithmic}
    \STATE {\bfseries Input:} data $x_i$, size $m$
    \REPEAT
    \STATE Initialize $noChange = true$.
    \FOR{$i=1$ {\bfseries to} $m-1$}
    \IF{$x_i > x_{i+1}$}
    \STATE Swap $x_i$ and $x_{i+1}$
    \STATE $noChange = false$
    \ENDIF
    \ENDFOR
    \UNTIL{$noChange$ is $true$}
  \end{algorithmic}
\end{algorithm}

==> algorithms/simulated-annealing.tex <==
\begin{algorithm}[ht]
\SetAlgoLined
\DontPrintSemicolon
\caption{Classic Simulated Annealing}
\label{alg:simulated_annealing}

\KwIn{Initial Solution $S_0$, Initial Temperature $T_{init}$, Cooling Rate $\alpha \in (0, 1)$, Stopping Temperature $T_{min}$}
\KwOut{Best Solution $S_{best}$}

$S \leftarrow S_0$\;
$S_{best} \leftarrow S$\;
$T \leftarrow T_{init}$\;

\While{$T > T_{min}$}{
    \tcp{Generate a neighbor candidate}
    $S_{new} \leftarrow \text{GenerateNeighbor}(S)$\;
    \tcp{Calculate energy change}
    $\Delta E \leftarrow E(S_{new}) - E(S)$\;

    \If{$\Delta E < 0$}{
        \tcp{Accept improvement (assuming minimization)}
        $S \leftarrow S_{new}$\;
        \If{$E(S_{new}) < E(S_{best})$}{
            $S_{best} \leftarrow S_{new}$\;
        }
    }
    \Else{
        \tcp{Accept worse solution with probability}
        $r \sim U(0, 1)$\;
        \If{$r < \exp(-\Delta E / T)$}{
            $S \leftarrow S_{new}$\;
        }
    }

    \tcp{Geometric cooling schedule}
    $T \leftarrow T \cdot \alpha$\;
}

\Return $S_{best}$\;
\end{algorithm}

==> bib/causality.tex <==
@inproceedings{chamberlain2021grand,
  title={Grand: Graph neural diffusion},
  author={Chamberlain, Ben and Rowbottom, James and Gorinova, Maria I and Bronstein, Michael and Webb, Stefan and Rossi, Emanuele},
  booktitle={International conference on machine learning},
  pages={1407--1418},
  year={2021},
  organization={PMLR}
}

==> cvlab-bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2}
 \else
   \parbox{#1}{#2}
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}
   \else
  \parbox{#1}{#2}
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3}
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}

==> cvlab-bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }







\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}

==> images/process_compare.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{images/process_compare_file.pdf}
    \caption{112}
    \label{fig:process_compare}
\end{figure}



==> tables/ablation_selected.tex <==
\begin{table}[ht]
\centering
\small
\caption{Ablation results on Split-A. \textit{Top}: comparison of \textit{In-Progress} schedule variants and consensus operators. \textit{Bottom}: thermodynamic parameter sensitivity (iterations $K$, heat height, sync windows). We report RMSD (\AA) and design-ipTM. Best performance is bolded.}
\label{tab:ablation_selected}
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Configuration}} & \multicolumn{3}{c}{\textbf{RMSD} (\AA) (\(\downarrow\))} & \multicolumn{3}{c}{\textbf{design-ipTM} (\(\uparrow\))} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & Ag. A & Ag. C & Avg. & Ag. A & Ag. C & Avg. \\
\midrule
\multicolumn{7}{l}{\small\textbf{\textit{Method Comparison}}} \\
Single-target \cite{boltzgen2025} & 4.11 & 3.85 & 3.98 & 0.18 & \textbf{0.21} & 0.20 \\
Greedy \cite{zhang2023diffcollage} & 4.45 & 4.48 & 4.47 & 0.17 & 0.19 & 0.18 \\
Greedy/w \cite{bar-tal2023multidiffusion} & 3.98 & 4.06 & 4.02 & 0.18 & 0.19 & 0.19 \\
Consistent  \cite{liu2022compositional} & 4.64 & 4.69 & 4.67 & 0.18 & 0.17 & 0.18 \\
Consistent /w & 4.46 & 4.41 & 4.44 & 0.18 & 0.19 & 0.19 \\
ACG & 3.75 & 3.78 & 3.76 & 0.19 & 0.20 & \textbf{0.20} \\
\rowcolor{red!8} ACG/w &\textbf{3.75} & \textbf{3.77} & \textbf{3.76} & \textbf{0.19} & 0.19 & 0.19 \\
\midrule
\multicolumn{7}{l}{\small\textbf{\textit{Exploration Depth (Iterations $K$)}} \cite{lugmayr2022repaint}} \\
$K=1$ & 3.76 & 3.77 & 3.76 & 0.19 & 0.19 & 0.19 \\
$K=2$  & \textbf{3.75} & \textbf{3.77} & \textbf{3.76} & \textbf{0.19} & \textbf{0.19} & \textbf{0.19} \\
$K=3$ & 3.88 & 3.95 & 3.92 & 0.19 & 0.19 & 0.19 \\
$K=4$ & 3.91 & 3.86 & 3.89 & 0.18 & 0.18 & 0.18 \\
\midrule
\multicolumn{7}{l}{\small\textbf{\textit{Noise Scale (Heat Height)}} \cite{song2019generative, song2020score}} \\
Height 1.00  & \textbf{3.75} & 3.77 & \textbf{3.76} & \textbf{0.19} & \textbf{0.19} & \textbf{0.19} \\
Height 0.75 & 3.88 & \textbf{3.72} & 3.80 & 0.19 & 0.19 & 0.19 \\
Height 0.50 & 3.83 & 3.78 & 3.80 & 0.19 & 0.19 & 0.19 \\
\midrule
\multicolumn{7}{l}{\small\textbf{\textit{Synchronization Windows}} \cite{yu2023freedom, bansal2024universal}} \\
Full Step Synchronization & 3.87 & 3.90 & 3.89 & \textbf{0.19} & 0.19 & 0.19 \\
Windowed Synchronization & \textbf{3.77} & \textbf{3.80} & \textbf{3.79} & 0.18 & 0.19 & \textbf{0.19} \\
No Synchronization & 4.14 & 4.01 & 4.07 & 0.18 & \textbf{0.20} & 0.19 \\
\bottomrule
\end{tabular}
\end{table}
